RankCSE: Unsupervised Sentence Representations Learning via Learning to Rank

Unsupervised sentence representation learning is one of the fundamental problems in natural language processing with various downstream applications. Recently, contrastive learning has been widely adopted which derives high-quality sentence representations by pulling similar semantics closer and pushing dissimilar ones away. However, these methods fail to capture the fine-grained ranking information among the sentences, where each sentence is only treated as either positive or negative. In many real-world scenarios, one needs to distinguish and rank the sentences based on their similarities to a query sentence, e.g., very relevant, moderate relevant, less relevant, irrelevant, etc. In this paper, we propose a novel approach, RankCSE, for unsupervised sentence representation learning, which incorporates ranking consistency and ranking distillation with contrastive learning into a unified framework. In particular, we learn semantically discriminative sentence representations by simultaneously ensuring ranking consistency between two representations with different dropout masks, and distilling listwise ranking knowledge from the teacher. An extensive set of experiments are conducted on both semantic textual similarity (STS) and transfer (TR) tasks. Experimental results demonstrate the superior performance of our approach over several state-of-the-art baselines.

==> figure_text/case_figure.tex <==
\begin{figure*}[t]
\centering

\begin{minipage}{0.38\linewidth}
\centering
\subfloat[KCC]{\includegraphics[width=0.5\textwidth]{figure/KCC.pdf}\label{fig:kcc}}
\subfloat[NDCG]{\includegraphics[width=0.5\textwidth]{figure/NDCG.pdf}\label{fig:ndcg}}
\captionof{figure}{Sentence representation performances on ranking metrics KCC and NDCG (detailed in Appendix \ref{ap:rank}). It can be seen that \gmodel captures more fine-grained ranking information than SimCSE \cite{DBLP:conf/emnlp/GaoYC21} and DiffCSE \cite{DBLP:conf/naacl/ChuangDLZCS0YKG22}.}
\end{minipage}
\hspace{0.1cm}
\begin{minipage}{0.60\linewidth}
\centering
\small
\tabcolsep=0.18cm
\begin{tabular}{p{4.6cm}ccc}
\toprule
\makecell[c]{\bf Sentences} & \bf Label & \bf SimCSE & \bf \gmodel \\
\midrule
$\bullet$ Broccoli are being cut by a woman & 4.80 (1) & 0.82 (2) & 0.95 (1)\\
$\bullet$ A woman is slicing vegetables & 4.20 (2) & 0.83 (1) & 0.91 (2) \\
$\bullet$ A woman is cutting some plants & 3.50 (3) & 0.74 (5) & 0.87 (3) \\
$\bullet$ There is no woman cutting broccoli & 3.40 (4) & 0.76 (3) & 0.85 (4)\\
$\bullet$ A woman is cutting some flowers & 2.87 (5) & 0.71 (7) & 0.81 (5) \\
$\bullet$ A man is slicing tomatoes & 2.60 (6) & 0.75 (4) & 0.79 (6) \\
$\bullet$ A man is cutting tomatoes & 2.40 (7) & 0.73 (6) & 0.76 (7) \\
\midrule
\multicolumn{4}{l}{\textbf{Input Sentence:} A woman is cutting broccoli} \\
\bottomrule
\end{tabular}
\captionof{table}{An example of an input sentence and seven other sentences from the STS datasets, with their similarity scores and rankings. The label scores are from human annotations. The SimCSE and \gmodel similarity scores are from the model predictions respectively, with the corresponding ranking positions. It can be seen that sentence rankings based on SimCSE are incorrect, while \gmodel generates more effective scores with accurate rankings.}
\label{tab:case}
\vspace{-3mm}
\end{minipage}
\end{figure*}

==> table/full_table.tex <==
\begin{table*}[t]
\small
\begin{adjustbox}{width=0.9\width,center}
  \begin{tabular}{p{2cm}|l|cccccccc}
    \toprule
     \bf PLMs & \bf Methods  & \bf STS12 & \bf STS13 & \bf STS14 & \bf STS15 & \bf STS16 & \bf STS-B & \bf SICK-R & \bf avg. \\
    \midrule
    \multirow{2}{*}{ Non-BERT} & GloVe(avg.) & 55.14 & 70.66 & 59.73 & 68.25 & 63.66 & 58.02 & 53.76 & 61.32 \\ 
    & USE & 64.49 & 67.80 & 64.61 & 76.83 & 73.18 & 74.92 & 76.69 & 71.22 \\
    \midrule
    \multirow{13}{*}{BERT$_{\rm base}$} & first-last avg. & 39.70 & 59.38 & 49.67 & 66.03 & 66.19 & 53.87 & 62.06 & 56.70 \\
    & +flow & 58.40 & 67.10 & 60.85 & 75.16 & 71.22 & 68.66 & 64.47 & 66.55 \\
    & +whitening & 57.83 & 66.90 & 60.90 & 75.08 & 71.31 & 68.24 & 63.73 & 66.28 \\
    & +IS & 56.77 & 69.24 & 61.21 & 75.23 & 70.16 & 69.21 & 64.25 & 66.58 \\
    & +CT & 61.63 & 76.80 & 68.47 & 77.50 & 76.48 & 74.31 &69.19 & 72.05 \\
    & +ConSERT & 64.64 & 78.49 & 69.07 & 79.72 & 75.95 & 73.97 & 67.31 & 72.74 \\
    & +SimCSE & 68.40 & 82.41 & 74.38 & 80.91 & 78.56 & 76.85 & 72.23 & 76.25 \\
    & +DCLR & 70.81 & 83.73 & 75.11 & 82.56 & 78.44 & 78.31 & 71.59 & 77.22 \\
    & +ArcCSE & 72.08 & 84.27 & 76.25 & 82.32 & 79.54 & 79.92 & 72.39 & 78.11 \\
    & +DiffCSE & 72.28 & 84.43 & 76.47 & 83.90 & 80.54 & 80.59 & 71.23 & 78.49 \\
    & \revise{+PaSeR} & 70.21 & 83.88 & 73.06 & 83.87 & 77.60 & 79.19 & 65.31 & 76.16 \\
    & +PCL & 72.84 & 83.81 & 76.52 & 83.06 & 79.32 & 80.01 & 73.38 & 78.42 \\
    & \bf +\gmodelnospace$_{\rm listNet}$ & \underline{74.38} & \underline{85.97} & \underline{77.51} & \underline{84.46} & \bf 81.31 & \underline{81.46} & \bf 75.26 & \underline{80.05} \\
    & \bf +\gmodelnospace$_{\rm listMLE}$ & \bf 75.66 & \bf 86.27 & \bf 77.81 & \bf 84.74 & \underline{81.10} & \bf 81.80 & \underline{75.13} & \bf 80.36 \\
    \bottomrule
\end{tabular}
\end{adjustbox}
\caption{Sentence representations performance of all baselines on STS tasks (Spearman's correlation). We directly import the results from the original papers and mark the best (bold) and second-best (underlined) results among models with the same PLMs. Results are statistically significant with p-value $<$ 0.005.}
\label{tab:full_stsr}
\end{table*}

\begin{table*}[t]
\small
\begin{adjustbox}{width=0.9\width,center}
  \begin{tabular}{p{2cm}|l|cccccccc}
    \toprule
    \bf PLMs & \bf Methods  & \bf MR & \bf CR & \bf SUBJ & \bf MPQA & \bf SST & \bf TREC & \bf MRPC & \bf avg. \\
    \midrule
    \multirow{2}{*}{Non-BERT} & GloVe(avg.) & 77.25 & 78.30 & 91.17 & 87.85 & 80.18 & 83.00 & 72.87 & 81.52 \\ 
    & Skip-thought & 76.50 & 80.10 & 93.60 & 87.10 & 82.00 & 92.20 & 73.00 & 83.50 \\
    \midrule
    \multirow{8}{*}{BERT$_{\rm base}$} & last avg. & 78.66 & 86.25 & 94.37 & 88.66 & 84.40 & \bf 92.80 & 69.54 & 84.94 \\
    & +IS & 81.09 & 87.18 & 94.96 & 88.75 & 85.96 & 88.64 & 74.24 & 85.83 \\
    & +SimCSE & 81.18 & 86.46 & 94.45 & 88.88 & 85.50 & 89.80 & 74.43 & 85.81 \\
    & +ArcCSE & 79.91 & 85.25 & \bf 99.58 & 89.21 & 84.90 & 89.20 & 74.78 & 86.12 \\
    & +DiffCSE$^\dagger$ & 81.76 & 86.20 & 94.76 & 89.21 & 86.00 & 87.60 & 75.54 & 85.87 \\
    & +PCL & 80.11 & 85.25 & 94.22 & 89.15 & 85.12 & 87.40 & 76.12 & 85.34 \\
    & {\bf +\gmodelnospace$_{\rm listNet}$} & \bf 83.21 & \underline{88.08} &  \underline{95.25} & \bf 90.00 & \bf 88.58 & \underline{90.00} & \underline{76.17} & \bf 87.33 \\
    & {\bf +\gmodelnospace$_{\rm listMLE}$} & \underline{83.07} & \bf 88.27 &  95.06 &  \underline{89.90} & \underline{87.70} &  89.40 &  \bf 76.23 &  \underline{87.09} \\
    \bottomrule
    \end{tabular}
\end{adjustbox}
\caption{Sentence representations performance of all baselines on transfer tasks (accuracy). The results of DiffCSE$^\dagger$ are obtained from the publicly available code and checkpoints for STS tasks, while others are imported from the original papers. We mark the best (bold) and second-best (underlined) results among models with the same PLMs. Results are statistically significant with p-value $<$ 0.005.}
\label{tab:full_tranr}
\end{table*}
